Evaluating Out-of-Distribution Performance on Document Image Classifiers

The ability of a document classifier to handle inputs that are drawn from a distribution different from the training distribution is crucial for robust deployment and generalizability. The RVL-CDIP corpus is the de facto standard benchmark for document classification, yet to our knowledge all studies that use this corpus do not include evaluation on out-of-distribution documents. In this paper, we curate and release a new out-of-distribution benchmark for evaluating out-of-distribution performance for document classifiers. Our new out-of-distribution benchmark consists of two types of documents: those that are not part of any of the 16 in-domain RVL-CDIP categories (RVL-CDIP-O), and those that are one of the 16 in-domain categories yet are drawn from a distribution different from that of the original RVL-CDIP dataset (RVL-CDIP-N). While prior work on document classification for in-domain RVL-CDIP documents reports high accuracy scores, we find that these models exhibit accuracy drops of between roughly 15-30% on our new out-of-domain RVL-CDIP-N benchmark, and further struggle to distinguish between in-domain RVL-CDIP-N and out-of-domain RVL-CDIP-O inputs. Our new benchmark provides researchers with a valuable new resource for analyzing out-of-distribution performance on document classifiers. Our new out-of-distribution data can be found at https://github.com/gxlarson/rvl-cdip-ood.

==> confusion.tex <==
\begin{table}[]
    \centering\scalebox{0.8}{
    \begin{tabular}{lllllllllllll}
        \textbf{Model}  & \rot{85}{\texttt{budget}}  
               & \rot{85}{\texttt{email}}
               & \rot{85}{\texttt{form}}
               & \rot{85}{\texttt{handwritten}}
               & \rot{85}{\texttt{invoice}}
               & \rot{85}{\texttt{letter}}
               & \rot{85}{\texttt{memo}}
               & \rot{85}{\texttt{news\_article}}
               & \rot{85}{\texttt{questionnaire}}
               & \rot{85}{\texttt{resume}}
               & \rot{85}{\texttt{scientific\_pub.}}
               & \rot{85}{\texttt{specification}}\\
    \midrule
       VGG-16 & 0.724 & 0.788 & 0.543 & 0.489 & 0.702 & 0.901 & 0.545 & 0.721 & 0.769 & 0.717 & 1.0 & 0.197 \\
       ResNet-50 & 0.672 & 0.424 & 0.514 & 0.415 & 0.561 & 0.836 & 0.576 & 0.651 & 0.692 & 0.505 & 1.0 & 0.164 \\
       GoogLeNet & 0.620 & 0.697 & 0.486 & 0.545 & 0.509 & 0.855 & 0.394 & 0.686 & 0.513 & 0.620 & 1.0 & 0.098 \\
       AlexNet & 0.483 & 0.667 & 0.471 & 0.472 & 0.632 & 0.861 & 0.455 & 0.663 & 0.513 & 0.543 & 1.0 & 0.148\\
       LayoutLMv2 & 0.897 & 0.848 & 0.514 & 0.273 & 0.333 & 0.842 & 0.424 & 0.500 & 0.744 & 0.560 & 1.0 & 0.180\\
       DiT & 0.862 & 0.970 & 0.914 & 0.665 & 0.877 & 0.954 & 0.667 & 0.849 & 0.821 & 0.739 & 1.0 & 0.410\\
       %CLIP & \\
    \bottomrule
    \end{tabular}}
    \caption{Per-class accuracy scores on RVL-CDIP-\textit{N} for each document classification model.}
    \label{tab:my_label}
\end{table}

==> confusion_matrices.tex <==
\begin{table}[]
    \centering
    \caption{Caption}
    \scalebox{0.65}{
    \begin{tabular}{lllllllllllllllll}
        & \rot{85}{\texttt{advertisement}} 
        & \rot{85}{\texttt{budget}}  
               & \rot{85}{\texttt{email}}
               & \rot{85}{\texttt{file\_folder}}
               & \rot{85}{\texttt{form}}
               & \rot{85}{\texttt{handwritten}}
               & \rot{85}{\texttt{invoice}}
               & \rot{85}{\texttt{letter}}
               & \rot{85}{\texttt{memo}}
               & \rot{85}{\texttt{news\_article}}
               & \rot{85}{\texttt{presentation}}
               & \rot{85}{\texttt{questionnaire}}
               & \rot{85}{\texttt{resume}}
               & \rot{85}{\texttt{scientific\_pub.}}
               & \rot{85}{\texttt{scientific\_report}}
               & \rot{85}{\texttt{specification}}\\
               \midrule
        \texttt{budget}             &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ 
        \texttt{email}              &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
        \texttt{form}               &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
        \texttt{handwritten}        &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
        \texttt{invoice}            &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
        \texttt{letter}             &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
        \texttt{memo}               &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
        \texttt{news\_article}      &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
        \texttt{questionnaire}      &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
        \texttt{resume}             &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
        \texttt{scientific\_pub.}   &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
        \texttt{specification}      &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
        \bottomrule
    \end{tabular}}
    \label{tab:idood_vgg16_confusion}
\end{table}

==> correlation.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{llllllll}
         & \rot{70}{VGG-16} & \rot{70}{ResNet-50} & \rot{70}{GoogLeNet} & \rot{70}{AlexNet} & \rot{70}{LayoutLMv2} & \rot{70}{DiT} & \rot{70}{CLIP} \\
    \midrule
        VGG-16     & 1.0  & 0.63 & 0.61 & 0.62 & 0.57 & 0.65 &  \\
        ResNet-50  &  & 1.0 & 0.58 & 0.57 & 0.57 & 0.58 &  \\
        GoogLeNet  &  &  & 1.0 & 0.56 & 0.54 & 0.57 &  \\
        AlexNet    &  &  &  & 1.0 & 0.55 & 0.56 &  \\
        LayoutLMv2 &  &  &  &  & 1.0 & 0.55 &  \\
        DiT        &  &  &  &  &  & 1.0 &  \\
        CLIP       &  &  &  &  &  &  &  \\
    \bottomrule
    \end{tabular}
    \caption{Pairwise similarity between predictions made by each model on RVL-CDIP-\textit{N}.}
    \label{tab:sim-scores-rvl-cdip-n}
\end{table}


\begin{table}[]
    \centering
    \begin{tabular}{llllllll}
         & \rot{70}{VGG-16} & \rot{70}{ResNet-50} & \rot{70}{GoogLeNet} & \rot{70}{AlexNet} & \rot{70}{LayoutLMv2} & \rot{70}{DiT} & \rot{70}{CLIP} \\
    \midrule
        VGG-16     & 1.0 & 0.45 & 0.43 & 0.44 & 0.42 & 0.27 &  \\
        ResNet-50  &  & 1.0 & 0.46 & 0.42 & 0.43 & 0.33 &  \\
        GoogLeNet  &  &  & 1.0 & 0.41 & 0.40 & 0.30 &  \\
        AlexNet    &  &  &  & 1.0 & 0.39 & 0.28 &  \\
        LayoutLMv2 &  &  &  &  & 1.0 & 0.30 &  \\
        DiT        &  &  &  &  &  & 1.0 &  \\
        CLIP       &  &  &  &  &  &  &  \\
    \bottomrule
    \end{tabular}
    \caption{Pairwise similarity between predictions made by each model on RVL-CDIP-\textit{O}.}
    \label{tab:sim-scores-rvl-cdip-o}
\end{table}
